Faster exact and approximation algorithms for packing and covering matroids via push-relabel

Matroids are a fundamental object of study in combinatorial optimization. Three closely related and important problems involving matroids are maximizing the size of the union of $k$ independent sets (that is, $k$-fold matroid union), computing $k$ disjoint bases (a.k.a. matroid base packing), and covering the elements by $k$ bases (a.k.a. matroid base covering). These problems generalize naturally to integral and real-valued capacities on the elements. This work develops faster exact and/or approximation problems for these and some other closely related problems such as optimal reinforcement and matroid membership. We obtain improved running times both for general matroids in the independence oracle model and for the graphic matroid. The main thrust of our improvements comes from developing a faster and unifying push-relabel algorithm for the integer-capacitated versions of these problems, building on previous work by Frank and Mikl\'os [FM12]. We then build on this algorithm in two directions. First we develop a faster augmenting path subroutine for $k$-fold matroid union that, when appended to an approximation version of the push-relabel algorithm, gives a faster exact algorithm for some parameters of $k$. In particular we obtain a subquadratic-query running time in the uncapacitated setting for the three basic problems listed above. We also obtain faster approximation algorithms for these problems with real-valued capacities by reducing to small integral capacities via randomized rounding. To this end, we develop a new randomized rounding technique for base covering problems in matroids that may also be of independent interest.

==> reinforcement.tex <==
\section{Minimum Cost Reinforcement}

\labelsection{reinforcement}    %


\newcommand{\minB}{B_0}
\providecommand{\cost}{\fparnew{c}}%


In this section we consider the minimum cost reinforcement problem. We
primarily discuss the more general matroid setting; the graphic
setting will follow immediately.

Our argument is closely tied to \citets{Cunningham1985c}{algorithm},
which was the first strongly polynomial time algorithm for this
problem. Here we describe the algorithm for the general matroid
setting.
\begin{enumerate}
\item Compute a maximum point $y \in \strength \ip$ subject to $y \leq x$.
\item Greedily extend $y$ to a base $y + z$ in $\strength \ip$, where
  $z \in \nnreals^{\groundset}$ as follows. Initially, we set
  $z(e) = 0$ for all elements $e$. Then for each element $e$ in
  increasing order of costs, set $z(e)$ large as possible subject to
  $y + z \in \ip$. The maximum value can be obtained by binary search,
  where each probe invokes matroid membership algorithm to see if the
  candidate value for $z(e)$ is feasible.
\end{enumerate}
We refer to \cite{Cunningham1985c} for the full justification of this
algorithm. Note that the algorithm requires many calls to a matroid
membership algorithm; first to compute the initial point $y$, and then
logarithmically many times for every element $e$ to obtain the right
$z(e)$.

Perhaps surprisingly, we show that the $k$-fold matroid union
push-relabel algorithm developed in \refsection{impr} also solves the
reinforcement problem in one shot. There is just one minor adjustment:
the initial base (which was allowed to be arbitrary) must be set to
the minimum cost base. Recall that the membership algorithm applied to
an input $x$ produces a maximum solution $\y$ and a point $\combox$ in
the base polytope, with $\y{e} = \min{\x{e}, \combox{e}}$. $y$
fulfills step 1 of \citets{Cunningham1985c}{algorithm}. It turns out,
as we prove below, that $\combox$ describes $y + z$ for an optimum
solution $z$; thus $z$ can be read off directly from $\combox$ and
$x$.  The overall running time, then, is exactly that of matroid
membership.  Here we have two speed ups compared to
\cite{Cunningham1985c} -- one from a faster membership algorithm, and
the second from omitting the second stage altogether. The following
lemma formalizes the key claim and implies the same running times as
$k$-fold matroid union for both general matroids and the graphic
matroid.

\begin{lemma}
  Let $\minB$ be the minimum cost base w/r/t $\cost$, and consider the
  exact push-relabel matroid membership algorithm adjusted so that the
  initial base is $\minB$. Let
  $\combo \in \simplex{\bases}$ be the
  convex combination of bases output by the push-relabel
  matroid-membership algorithm.  Define
  $z \in \nnreals^{\groundset}$ by
  \begin{align*}
    z(e) = \min{0, \combox{e} - \x{e}} \text{ for } e \in \groundset.
  \end{align*}
  Then $z$ is a minimum cost reinforcement.
\end{lemma}

\begin{proof}
  Without loss of generality we assume $\strength = 1$.  Let $\combo$
  and $\level$ be the convex combination and levels, respectively,
  produced by the algorithm.  Let
  $C = \setof{e \where \combox{e} > \x{e}}$. We have $\level{e} = 0$
  for all $e \in C$ by invariant \ref{mm-level-0}.
  \begin{claims}
  \item $C \subseteq \minB$.
  \end{claims}
  To this end, observe that initially we have $\combox{e} > \x{e}$
  only for elements in the initial base, $e \in \minB$. Thereafter, a
  coordinate $\combox{e}$ is only increased if $\combox{e} < \x{e}$,
  and never exceeding $\x{e}$.

  \begin{claims}
  \item \labelclaim{mcr-claim-2} For any element $e \in \minB$, and
    any base $B' \in \support{\combo}$, we have either $e \in B'$, or
    $e \in \spn{B' \setminus C}$.
  \end{claims}
  Fix any element $e \in \minB$. Throughout the algorithm, $e$ is
  removed from a base $B'$ in $\combo$ only if it is replaced by an
  element $d$ one level higher, such that
  $B'_{\geq \level{d}} = B'_{> \level{e}}$ spans $e$. Thus at
  termination, for every base $B' \in \support{\combo}$, if
  $e \notin B'$, then $e \in \spn{B'_{> 0}}$. Since $C \subseteq L_0$,
  we have $B'_{> 0} \subseteq B' \setminus C$, hence
  $e \notin \spn{B' \setminus C}$.

  Now, let $y = \combox \cap \capacity$; $y$ is a base in
  $P/\capacity$.  Recall that any minimum cost basis can be produced
  by a greedy algorithm adding feasible elements in nondecreasing
  order of cost.  Number the elements
  $\groundset = \setof{e_1,e_2,\dots}$ in nondecreasing order of cost,
  breaking ties so that the greedy algorithm processing elements in
  this order produces $\minB$. In Cunningham's algorithm, a minimum
  cost reinforcement $z$ is obtained by processing the $e_i$'s in
  order, taking setting $z(e_i)$ to the maximum quantity subject to
  $y + z \in P$. (This equals the minimum quantity subject to $y+z$
  spanning $e_i$, and in Cunningham's algorithm it is identified via
  binary search and matroid membership).  Let us call this
  ``Cunningham's greedy augmentation'', which Cunningham has already
  shown to be optimal. The following claim would thus complete the
  proof.
  \begin{claims}
  \item Cunningham's greedy augmentation selects
    $z(e) = \max{\combox{e} - \x{e}, 0}$ for all $e \in \groundset$.
  \end{claims}

  We analyze each element in the greedy order.  Consider the $i$th
  iteration (where $i \in [n]$), in which the greedy algorithm
  processes $e_i$. We assume by induction that $y + z$ spans
  $\setof{e_1,\dots,e_{i-1}}$. (The base case, where $i = 1$, holds
  vacuously.) If $e_i \notin \minB$, then
  $e_i \in \spn{e_j \in \minB \where j < i}$, so $e_i$ is spanned by
  $y+z$. If $e_i \in \minB$, then we claim that the greedy algorithm
  sets $z(e_i) = \combox{e_i} - \x{e_i}$. Let $z'$ be the vector
  obtained from $z$ by setting $z'(e_i) = \combox{e_i} - \x{e_i}$. On
  one hand $y + z'$ is feasible because $y + z' \leq \combox$. On the
  other hand, $y+z'$ contains the convex combination of independent
  sets,
  \begin{align*}
    \sum_{B'} \combo{B'} \cdot \ones_{B'
    \setminus (C-e)}.
  \end{align*}
  By \refclaim{mcr-claim-2}, for every $B' \in \support{\combo}$, the
  set $B' \setminus (C-e)$ spans $e$, hence $y+ z'$ spans $e$. This
  shows that algorithm takes $z(e_i) = \combox{e_i} - \x{e_i}$. This
  establishes the claim, and completes the proof.
\end{proof}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:

